Fully Automated Shape Analysis Based on Forest Automata

Forest automata (FA) have recently been proposed as a tool for shape analysis of complex heap structures. FA encode sets of tree decompositions of heap graphs in the form of tuples of tree automata. In order to allow for representing complex heap graphs, the notion of FA allowed one to provide user-defined FA (called boxes) that encode repetitive graph patterns of shape graphs to be used as alphabet symbols of other, higher-level FA. In this paper, we propose a novel technique of automatically learning the FA to be used as boxes that avoids the need of providing them manually. Further, we propose a significant improvement of the automata abstraction used in the analysis. The result is an efficient, fully-automated analysis that can handle even as complex data structures as skip lists, with the performance comparable to state-of-the-art fully-automated tools based on separation logic, which, however, specialise in dealing with linked lists only.

==> normal_forms.tex <==
\todo{
\paragraph{Normal forms and interconnection equivalence of graphs}
\begin{itemize}
\item
This could be probably moved elsewhere, inclusion is not important in this paper. Probably somewhere close to where the connection between knot in the interconnection and a knot in a graph is introduced.
\item
two graph are interconnection equivalent / have equivalent interconnection, iff there is a bijection $f$ from $\cpsof\graph$ to $\cpsof\graphprime$ such that
\begin{itemize}
\item
$f$ respects ports,
\item
$f$ respects spans, and
\item
a double path from $c$ to $c'$ in $\graph$ shares an edge with a double from $d$ to $d'$ iff
a double path from $f(c)$ to $f(c')$ in $\graph'$ shares an edge with a double path form $f(d)$ to $f(d')$ in $\graphprime$.
\end{itemize}
\item
a double path (trace?) is defined as something like two straight paths (from and to some node $v$) in some where one of them might be empty
\item
a forest automaton is interconnection uniform if all its graph have equivalent interconnection.
\item
we can split a FA into several ones with uniform interconnection, in the tech. rep., not enough space, not enough people, ...
\item
(you can thus pick any graph from the language as a representative. Good to pick a small one, how?)
\end{itemize}
}
%-------------------------------------------------------------------------------
\vspace*{-2mm}\paragraph{Normal forms and skeletons of graphs.}\label{sec:canonical}
%-------------------------------------------------------------------------------
We call an io-forest $\forest = (\trees,\fports)$ \emph{minimal} iff the roots
of the trees $\trees$ are the cut-points of $\otimes \forest$. A~minimal forest
representation of a graph is unique up to reordering of $\trees$. 
Let the \emph{canonical ordering} of cut-points of $\otimes\forest$ be defined by the cost of the cheapest paths leading from the input port to them. 
We use $\cpof{\otimes\forest} i$ to denote the $i$-th cut-point in this ordering. 
We say that
$\forest$ is \emph{canonical} iff it is minimal, $\otimes \forest$ is
accessible, and the trees within $\trees$ are ordered by the canonical ordering of their roots (which are cut-points of $\otimes\forest$).
A~canonical forest is thus a unique representation of an accessible io-graph.
We say that a~FA \emph{respects canonicity} if all forests from its forest
language are canonical. Respecting canonicity makes it possible to efficiently
test FA language inclusion by testing TA language inclusion of the respective
components of two FA. This method is precise for flat FA and sound (not always
complete) for FA of a higher level \cite{forester11}.

Next, we discuss a concept strongly related to canonicity, which is the notion
of skeletons of graphs. 
We say that a path in an io-graph $\iograph$ is \emph{straight} iff it is simple and none of its inner node is a
cut-point.
We define the \emph{span} of a node $u\in\domof \graph$ in $\iograph$ as a 
sequence $\spanof \iograph u = v_1\cdots v_n\in \cpsof\iograph^{*}$ which contains one
occurrence of every node of $\cpsof\iograph$ reachable by exactly one straight path from
$u$ and two occurrences of $v$ if it is reachable by multiple straight paths. The nodes
$v_1\cdots v_n$ are ordered according to the costs of the cheapest paths
leading from $u$ to them (multiple occurrences of the same node are therefore
next to each other). The \emph{skeleton} of $\iograph$ is the io-graph $\cigof \iograph = (\{\edgeof u \Box
{\spanof \iograph u}\mid u\in \cpsof\iograph\}, \gports)$. It records reachability (and multiple
reachability) between all cut-points of $\iograph$. 

\begin{wrapfigure}[9]{r}{25mm}
\begin{center}
\vspace{-15mm}
\figswitch{
\input{figs/igraph.tikz}
}
\vspace{-4mm}
\caption{An io-graph $\iographof \graph 1$ and $\cigof{\iographof \graph 1}$.}
  \label{fig:igraph}
\end{center}
\vspace{-8mm}
\end{wrapfigure}

Fig.~\ref{fig:igraph} shows an io-graph with the input port $1$ and its skeleton $\cigof {\iographof \graph 1}$.
The skeleton $\cigof {\iographof \graph 1}$ has the domain $\{1,2,3\}$ of cut-points of $\graph$,  
which are connected (cf.~the dashed edges) iff they are connected in $\graph$, and they are connected by two edges iff they are connected by multiple straight paths in $\graph$.
(The highlighted area is explained in~Sect.~\ref{sec:knots}.)

%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
\enlargethispage{8mm}
%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!

We call a~FA $\fa$ \emph{state uniform} iff each of its component TA $\ta$ has
a single root state and all nodes of all graphs accepted by the same state $q$
of $\ta$ have equivalent spans (i.e., they reach equivalent
cut-points, in the same order, and with the same multiple reachability). 
That is, there exists a sequence of numbers $\qspanof q = i_1\cdots i_n$ such that for every node $v\in\domof\graph$ of an io-graph $\iograph\in\langof\fa$, which is labelled by
$q$ in an accepting run of $\fa$, $\spanof \iograph v = \cpof \iograph {i_1} \cdots \cpof \iograph {i_n}$. 
Graphs accepted by a state uniform FA $\fa$ have isomorphic skeletons (identical up to naming of nodes). 
We will pick from the isomorphic skeletons a unique representative as a skeleton of $\fa$ as that one where the cut-points are identified with their positions in the canonical cut-point ordering.
Formally, we define the \emph{skeleton of a state uniform FA $\fa$}, denoted $\cigof\fa$, as $\cigof\iograph$ where $\iograph\in\langof\fa$ and $\cpof \iograph i = i$ for all $1\leq i\leq |\cpsof\graph|$.

State uniform FA respect canonicity as discussed in \cite{forester11}, which
also gives a procedure for transforming a given FA into a \emph{set} of state
uniform---and hence canonicity respecting---FA (FA are not closed under union,
and so the obtained FA cannot be in general united into one FA).
State uniformity also
simplifies the procedure of box learning and folding as presented further.  

%\clearpage



==> old_stuff.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace*{-2mm}\section{Learning of Boxes}\label{sec:learning}\vspace*{-1mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As we have already mentioned, sets of graphs with an unbounded number of can only 
be described by FA with a help of boxes used to turn joins into ordinary
nodes only. In particular, boxes allow subgraphs with multiple paths leading into a join to be
replaced by a single edge, and hence to decrease the in-degree of the join. When
the in-degree drops to 1, the join turns into an ordinary node.

We head towards an operation of folding a~FA $\fa$
which should result in an automaton $\fa'$ where $\semof\fa = \semof{\fa'}$ and a box $B$ that encodes a set of subgraphs of graphs from $\langof\fa$. $B$ acts as a sub-label of the graphs of $\langof{\fa'}$. 
Graphs of $\langof{\fa'}$ have either smaller number of joins or at least smaller sum of in-degrees of joins than the graphs of $\langof\fa$.

%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
\enlargethispage{6mm}
%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!

%===============================================================================
\vspace*{-2mm}\subsection{Knots of Graphs}\label{sec:knots}\vspace*{-1mm}
%===============================================================================
Before we come to the details of the technique of folding FA, 
we discuss the criteria that should be satisfied by subgraphs of graphs of $\langof\fa$ which are to be folded into the box $B$.
Generally speaking, the strategy for picking folded subgraphs should allow eliminating a large (possibly unbounded) number of joins with a small number of boxes. The folded subgraphs should therefore contain input sub-edges of joins, but should be also small and simple in order to be reusable.
\todo{
More particularly, 
a box is usefull if it can be used unboundedly many times to eliminate a join.
Moreover, the occurences must be such that the box is not incident with any other join, otherwise we still have the problem of unboundedlty many joins. 
%
Hierarchy:
Knots within knots.
The knot with more joins is more likely to belong to a higher hierarchy level.
What does this mean?
}
%
Let us first give some necessary definitions.
%

A graph $\graphprime$ is a \emph{subgraph} of a graph $\graph$, denoted as $\graphprime \subgrapheq \graph$, iff $\gsedgesof{\graphprime} \subseteq \gsedgesof{\graph}$. 
%
The \emph{border} of $\graph'$ in $\graph$
%, denoted $\borderof {\graph'} \graph$, 
is the subset of nodes of 
$\domof{\graph'}$
that are connected with nodes in $\domof{\graph}\setminus\domof{\graph'}$ 
by an incoming or an outgoing edge. 
%
%In the context of subgraphs, it will be advantageous to talk about sequences of sub-edges that correspond to paths. 
A \emph{trace} from a node $u$ to a node $v$ in a graph $\graph$ is a sequence of sub-edges $\sedge_0\cdots\sedge_n\in\gsedgesof\graph^*$ such that $n \geq 0$, $\sedge_0$ is an outgoing
sub-edge of $u$, $\sedge_n$ is an incoming sub-edge of $v$, and for all $1\leq
i \leq n$, 
%there is a successor $w$ of $\edge_{i-1}$ such that $\edge_i$ is an outgoing sub-edge of $w$.
the origin of $\edge_i$ is one of the targets of $\edge_{i-1}$.
Analogically as for paths, we call the origin of $\edge_1\cdots\edge_n$ the \emph{inner nodes} of the trace. 
Let $\iograph$ be an io-graph. We define a \emph{straight trace} of
$\iograph$ as a trace of $\graph$ where no inner node appears twice as a
origin of a sub-edge and no inner node is a cut-point of $\iograph$.
%
%For a set of nodes $V$, we define a $V$-straight trace of $\graph$ 
%as a trace of $\graph$ where no inner node appears twice as a
%origin of a sub-edge and no inner node is in $V$.
%Given an io-graph $\iograph$, a straight trace of $\iograph$ is a $\cpsof\iograph$-straight trace of $\graph$.
%
Let $\graphprime$ be a subgraph of $\graph$. The \emph{closure} of $\graphprime$ is the smallest (w.r.t. $\subgrapheq$) graph $\hgraph$ with $\graph'\subgrapheq\hgraph\subgrapheq\graph$ such that for any distinct
$u,v\in\domof\graphprime$: 
%\begin{enumerate}[(i)]
\begin{inparaenum}[(i)]
  \item\label{enum:one_path} 
$\gsedgesof\hgraph$ contains every straight trace $\trace$ of $\iograph$ from $u$ to $v$, and
  \item\label{enum:two_paths} 
    for every pair of straight traces $\trace_1$ and $\trace_2$ of $\iograph$ with disjoint sets of inner nodes from a node $n \in \domof{\graph}$ to $u$ and $v$, respectively, $\gsedgesof\hgraph$ contains both $\trace_1$ and $\trace_2$.
%\end{enumerate}
\end{inparaenum}

For the rest of Section~\ref{sec:knots}, let us fix an io-graph $\iograph\in\langof\fa$.
In the next paragraph, we will introduce the notion of knot 
which summarises desired properties of a subgraph $\knot$ of $\graph$ 
such that $\iographof\knot\gportsprime\in\langof B$ for some sequence of ports $\gportsprime$.
The subgraph $\knot$ is to be folded, i.e., replaced by a single sub-edge $\sedge$ labelled by $B$, which gives rise to an io-graph $\iographof \graphprime\gports\in\langof{\fa'}$ with
$\graph = \graph'\subst{\iographof \knot \gportsprime}{\sedge}$.

%The properties are summarised by the notion of knot, defined below.

%If the symbol $a$ above is a~FA and $\iographof {\graph'} \gports \in L(a)$, we say that
%$\hgraph = \graph\subst{\iographof {\graph'} \gports}{\ithedgeof i}$ is an \emph{unfolding} of
%$\graph$, written $\graph\unfold\hgraph$. Conversely, we say that $\hgraph$
%arises from $\graph$ by \emph{folding} $\iographof {\graph'} \gports$ into $\ithedgeof i$. 


%\end{inparaenum}

%-------------------------------------------------------------------------------
\vspace*{-1.5mm}\paragraph{Knots.}
%-------------------------------------------------------------------------------

%The criteria that we see as the most crucial for selecting subgraphs to be folded are the following. 
%We are now ready to define the notion of \emph{knot} of a graph, a subgraph of the graph which is a candidate for folding.
%$\graph'$ be the graph that arises from a graph $\graph$ by
%folding an io-graph $(\hgraph,\gports)$ into $\etermof  v i$. 
%give the basic criteria for subgraphs of a graph to be folded. 
%\begin{definition}
\todo{
(Define a knot of size $n$ inductivelly....)
A minimal knot $\knot$ of $\graph$ is a minimal subgraph of $\graph$ which contains a cycle or two paths from a node $u$ to a node $v$ (with disjoint sets of inner nodes). 
It does not contain ports.
%
The size / complezity of a minimal knot is $|\joinsof\graph\cap\domof\knot|$.
The set $|\joinsof\graph\cap\domof\knot|$ is called the signature of the knot.
Every minimal knot of a size $n$ is a knot of size $n$.
The union of two knots of size $n$ who share a sub-edge is also a knot of size $n$.
%
An optimal knot of size $n$ is a union of maximal knots of size $n$ with the same signature. It has a source and is not incident with any port.
}

We define \emph{knot} of $\iograph$ as a subgraph $\knot$ of $\graph$ that has the following properties:
%\begin{enumerate}[(i)]
\begin{inparaenum}[(1)]
  \item\label{enum:contains_join} 
it contains a~join or a~cycle,
  \item\label{enum:has_source}
it is accessible from a node $\src\in\domof\knot$, called a \emph{source}, which is itself reachable from $\gport_1$ by a trace $t$ such that no sub-edge of $t$ is in $\gsedgesof\knot$,
  \item\label{enum:contains_closure}
it equals its own closure,
  \item\label{enum:no_cutpoints} 
%$\domof\knot$ does not contain any port from $\gports$,
it does not contain ports of $\iograph$,
%\end{enumerate}
\end{inparaenum}
%\end{definition}
\medskip

\begin{wrapfigure}[4]{r}{0.31\textwidth}
%\begin{center}
\vspace{-9mm}
\figswitch{
\input{figs/wurst_fork.tikz}
\input{figs/wurst_cycle.tikz}
}
\vspace{-2mm}
  \caption{Knot, Property~\ref{enum:contains_join}.}\label{fig:knot}
%\end{center}
\end{wrapfigure}

The individual properties of the definition are motivated by the following:
Property~\ref{enum:contains_join} is necessary from the very basic reason why we introduce knots: to eliminate joins by folding them. A join can be eliminated from $\graph$ by folding $\knot$ in two ways: (a) if it is completely removed from $\graph$, or (b) if its in-degree is decreased to 1. Both cases are possible only if either (i) the join appears in $\knot$ with the in-degree more than 1, which means that it is a join of $\knot$, or (ii) if $\knot$ contains a cycle through the join (in this case, the join is not necessarily a join of $\knot$). Fig.~\ref{fig:knot} shows two knots. Highlighted are their smallest subgraphs satisfying Property~\ref{enum:contains_join} which are in fact minimal (w.r.t. $\subgrapheq$) knot. 

\begin{wrapfigure}[9]{r}{27mm}
\vspace{-6mm}
\hspace*{-6mm}
\begin{subfigure}{0.3\textwidth}
 \centering
{
\figswitch{
 \input{figs/sll_tail_ptr.tikz}
}
 \caption{SLL with tail ptrs.}
 \label{fig:tail_ptrs}
 }
\end{subfigure}
\hspace*{-6mm}
\begin{subfigure}{0.3\textwidth}
 \centering
{
\figswitch{
 \input{figs/sll_head_ptr.tikz}
}
 \caption{SLL with head ptrs.}
 \label{fig:head_ptrs}
 }
\end{subfigure}
  \vspace{-3mm}
  \caption{Closure.}
 % \label{fig:optimal}
%\end{center}
\end{wrapfigure}
Property~\ref{enum:has_source} implies together with Property~\ref{enum:contains_join} that $\graph'$ has indeed a smaller sum of in-degrees of joins than $\graph$. 
Besides that
%, it is important for preserving accessibility of $\graph$. i.e., 
it guarantees that if $\iograph$ is accessible, then $\iographof \graphprime\gportsprime$ is accessible, and vice versa. It also guarantees accessibility of $\knot$ itself, which is a necessary condition for existence of a canonic forest representation.

%Property~\ref{enum:contains_closure} enforces knots to be not ``too small'' due to points 
%\ref{enum:one_path} and \ref{enum:two_paths} of the definition of a closure.
Property~\ref{enum:contains_closure} prevents us from folding ``too small'' subgraphs in the following sense. 
Assume that $\knot$ does not contain its closure.
Then, by definition, there are nodes $u$ and $v$ of $\knot$ and either (i) a straight trace $\trace$ from $u$ to $v$ leading outside $\knot$, 
or (ii) a node $n$ outside $\knot$ with two non-crossing straight traces $\trace_1,\trace_2$ from $n$ to $u$ and to $v$, respectively.
Both scenarios are shown in Fig.~\ref{fig:how_wurst_got_its_name}.
In both situations, some nodes of $\knot$ will still be joins even in the graph $\graph'$ (which arises from $\graph$ after folding $\knot$ into a sub-edge $\sedge$). The only way of eliminating all joins appearing in $\knot$ from $\graph$ is to fold $\knot$ together with the trace $\trace$ (in case (i)), or with traces $\trace_1,\trace_2$ (in case (ii)).
Let us look closer for instance at the case (i), when there is a straight trace $\trace$ from $u\in\domof\knot$ to $v\in\domof\knot$ leading via the outside of $\knot$. We will argue that in the graph $\graph'$, $v$ or another node of $\knot$ is still a join. Node $v$ must be an origin or a target of the sub-edge $\sedge$ that in $\graph'$ replaces $\knot$ since it is an element of the border of $\knot$ in $\graph$. In case it is a target, it is a join of $\graph'$ since it has two incoming sub-edges: $\edge$ and the last sub-edge of $\trace$. In case it is the origin of $\edge$ and also a source of $\knot$, it has two incoming sub-edges too: the last sub-edge of $\trace$ and the last sub-edge of a trace from $\gports_1$ (which exists by the definition of source of $\knot$). Last, in case $v$ is the origin of $\edge$ but not a source of $\knot$, then there is another source $\src$ of $\knot$ (by Property~\ref{enum:has_source} of the definition of knot) which is still a join of $\graph'$ since it is reachable from outside $\knot$ and also by $\sedge$. Overall, it can be shown this way that in order to eliminate all joins of $\graph$ that appear within $\knot$, $\knot$ must be folded together with $\trace$.  
Point~(ii) of the definition of closure can be jutified by a similar reasoning as the above. 
%

Next, we give an example of a practical situation where Property~\ref{enum:contains_closure} prevents infinite diverging sequence of folding which coud arise if to small subgraphs were folded. 
Consider for example a minimalistic strategy that always picks the smallest subgraph such that folding it decreases the sum of in-degrees of joins.  
This strategy is shown impractical when applied to the set of all lists with tail pointers. 
As illustrated in Fig.~\ref{fig:tail_ptrs}, it generates an infinite hierarchy of knots, each enclosing a list of one particular length in the form of the head connected to a knot encoding the tail. Since FA do not allow recursive nesting of boxes, the hierarchy could be encoded only using an infinite number of boxes.
This undesired behaviour of folding is prevented by the Property~\ref{enum:two_paths} of closure that enforces that only an entire list can be picked as a knot. 
The set of all such lists (knots) can be then encoded as a~FA and folded into a single box. 
A mirror problem arises when using the minimalistic strategy to fold lists with head pointers, as illustrated in Fig.~\ref{fig:head_ptrs}. In this case, Property~\ref{enum:one_path} of a closure enforces that only an entire list can be picked as a knot and all lists can be then folded into a single box.

The last property~\ref{enum:no_cutpoints}, is in fact not strictly compulsory, but is included for simplicity. Ports could be parts of knot if they were treated in a special way.
However, since there is only a fixed number of ports ports cannot be eliminated from an io-graph by folding anyway, foding them into boxes is not necessary.
%Finally, Point~\ref{enum:no_cutpoints} is required since ports can never stop being cut-points due to folding. 
%, which is not a problem since there is always only a fixed number of them.

%-------------------------------------------------------------------------------
\vspace*{0mm}\paragraph{Detection of minimal knots.}
%-------------------------------------------------------------------------------
\todo{Equivalence $f$ defines an equivalence (bijection) between optimal knots.
The equivalence maps joins to their $f$ images, maps the source to the corresponding fork whicih is also the source, and takes all tree segments between these nodes.
%
Lemma - if one is optimal, then the other is (works with $f^{-1}$ too, does it matter?)
}

In order to achieve maximal reusability of boxes, we pick for folding knots
which are among knots of $\iograph$ minimal w.r.t. $\subgrapheq$.
%(in fact, sometimes we need to additionally extend the minimal knots found, as discussed later).
In this paragraph, we discuss how minimal knots of $\iograph$ can be
identified using the skeleton of $\iograph$. This will give
a basis for a procedure for folding a set of minimal knots of io-graphs from
$\langof\fa$ into a box using the skeleton of $\fa$, described in
detail in Section~\ref{sec:folding_overview}.

\begin{wrapfigure}[9]{r}{32mm}
\vspace{-14mm}
\begin{center}
\figswitch{
\hspace{-0mm}\parbox{26mm}{\input{figs/root_ptr_tree.tikz}}\\
}
%\parbox{5mm}{\vspace{-12mm}\input{figs/cig_root_ptr_tree.tikz}}\\
\vspace{-2mm}
  \caption{A tree with root pointers and its skeleton}
  \label{fig:tree_root_ptrs}
\end{center}
\end{wrapfigure}
%
%Given a knot $\knotprime$ of $\cigof\iograph$, 
%an \emph{interpretation} of $\knotprime$ in $\iograph$ is a knot $\knot$ of
%$\iograph$ with the following properties: 
%%
%\begin{inparaenum}[\itshape a\upshape)]
%  \item  \label{enum:interpretation_trace_for_path}  for every pair of nodes
%    $u,v\in\domof\graph$ such that there is an edge from $u$ to $v$ in
%    $\knotprime$, $\knot$ contains a straight trace from $u$ to $v$, and
%  \item  no proper subgraph of $\knot$ is a knot with
%    Property~\ref{enum:interpretation_trace_for_path}.
%\end{inparaenum}
Given a knot $\knotprime$ of $\cigof\iograph$, 
an \emph{interpretation} of $\knotprime$ is a minimal subgraph $\interp$ of $\graph$ such that
\begin{inparaenum}[\itshape a\upshape)]
  \item $\interp$ is a knot of $\iograph$, and
  \item  \label{enum:interpretation_trace_for_path}  for every pair of nodes
    $u,v\in\domof\graph$ such that there is an edge from $u$ to $v$ in
    $\knotprime$, $\interp$ contains a straight trace from $u$ to $v$.
\end{inparaenum}
%
%
%contains one straight path from $$\gsedgesof\knot$ contains all straight traces of $\iograph$ between nodes of $\knotprime$.
%$u \mapsto (\Box, v_1 \dots v_n)$ in $\knotprime$ there is for every $v_i \in
%\{v_1, \dots, v_n\}$ a straight path from $u$ to $v_i$ in $\knot$.

The example in
Fig.~\ref{fig:tree_root_ptrs} of a tree with root pointers illustrates that there may be more then one interpretations of $\knotprime$. The knot in the skeleton, consisting of the node $\bullet$ and a self-loop on the node, gives
rise to 3 different knots in the original shape.

%By the definitions of a knot, a skeleton, and an interpretation, 
%$\interp$ must be accessible from a source $\src$ of $\knotprime$.
The interpretation $\interp$ is not neccesarily a \emph{minimal} knots of $\iograph$. 
We will show that in such a case, it contains a unique minimal knot of $\iograph$ which can be algorithmically extracted.
Let $\src$ be a source of $\interp$. 
We define the \emph{fork point} of $\interp$ from $\src$ as the node 
$\forkof \interp \src\in\domof{\interp}$ that equals $\src$ in case there is a cycle through $\src$ in $\interp$, and otherwise it is the node such that
all straight traces from $\src$ to 
$\cpsof{\iograph}$ 
%that are in $\interp$ 
traverse it,
and no successor of $\forkof \interp \src$ in $\interp$ has this property. 
For a source $\src$ of $\interp$ such that $\src\neq\forkof \interp \src$, we call a straight trace from $\src$ to $\forkof \interp \src$ an \emph{access trace of $\interp$}.
%If define an \emph{access trace} of $\interp$ is a straight trace from a source $\src$ such that $\src \neq \forkof \interp \src$ to $\forkof \interp \src$.

%\begin{figure}[ht]
%  \centering
%\figswitch{
%  \input{figs/fork.tikz}    % forgot to commit [Ondra]
%}
%  \caption{beautiful figure }
%  \label{fig:interpretation}
%\end{figure}

%Note that $\forkof{\graph}{u}{V}$ may be undefined if there are no straight
%paths from $u$ to $V$.
%
%\begin{lemma}\label{lemma:single_path}
%  Given a graph $\graph$, a set of nodes $V \subseteq \domof{\graph}$ and
%  a node $u \in \domof{\graph}$, if $\forkof{\graph}{u}{V}$ is defined then
%  either $u = \forkof{\graph}{u}{V}$ or there is exactly one straight path
%  from $u$ to $\forkof{\graph}{u}{V}$.
%\end{lemma}
%
\begin{lemma}\label{lemma:single_path}
  An interpretation of a minimal knot of $\cigof\iograph$ has at most one access trace.  
\end{lemma}
%
%\begin{proof}
%  First, consider the case when there are multiple sources in $\knot$.
%  Let us consider two distinct sources $\src, \srcprime \in \domof{\knot}, \src \neq \srcprime$.
%  From the definition of a source, $\src$ and $\srcprime$ are mutually
%  reachable, which means that there must be a cycle through $\src$ (and also
%  through $\srcprime$).
%  Therefore, for every source $\src$ of $\iograph$ it holds that $\src
%  = \forkof{\knot}{\src}$ so there is no access trace in $\graph$.
%
%  Second, for the case when there is a single source $\src$ in $\knot$ it
%  either holds that $\src = \forkof{\knot}{\src}$, in which case there is
%  again no access trace in $\knot$, or $\src \neq f = \forkof{\knot}{\src}$.
%  We prove the presence of exactly one access trace for the latter case by
%  contradiction.
%  Suppose that there are two straight traces from $\src$ to $f$.
%  The sets of inner nodes of these traces need to be disjoint (otherwise they
%  would contain a cut-point and would not be straight).
%  Therefore, $f$ is a cut-point of $\iograph$ and $f$ occurs twice as
%  a~successor of $\src$ in $\cigof{\iograph}$.
%  We further know that $\src$ is not in a cycle in $\knot$ (otherwise there would be
%  multiple sources in $\knot$) and that there is no path from $\src$ to any
%  other cut-point of $\knot$ not traversing $f$ (from the definition of
%  $\forkof{\graph}{\src}$).
%  Therefore there is a knot in $\cigof{\iograph}$ that contains only the nodes
%  $\src$ and $f$, which is smaller than $\knotprime$, which is a contradiction
%  because $\knotprime$ is minimal.
%  \qed
%\end{proof}

For an interpretation $\interp$ of a minimal knot $\knotprime$ of $\cigof{\iograph}$, we call the \emph{core} of $\interp$ the knot $\coreof{\interp}$ which is defined by $\gsedgesof{\coreof{\interp}}
= \gsedgesof{\interp} \setminus \{e_1, \dots, e_n\}$ where $e_1 \cdots e_n$ is the
access trace of $\interp$ if it exists, otherwise it is the empty sequence.
We say that the graph $\coreof{\interp}$ is \emph{induced} by $\knotprime$.
It follows from Lemma~\ref{lemma:single_path} that there is
exactly one core of a particular interpretation of a minimal knot of $\cigof\iograph$.
%We say that the minimal knots of $\iograph$ are \emph{induced} by $\knotprime$.
\begin{lemma}\label{lemma:minknot_induces_minknot}
%VERSION 1
%If $\knotprime$ is a minimal knot of $\cigof{\iograph}$ and $\interp$ is its
%interpretation, then $\coreof{\interp}$ is a minimal knot of
%$\iograph$.
%
%VERSION 2
%Let $\interp$ be an interpretation of a minimal knot of $\cigof\iograph$.
%Then $\coreof\interp$ is a minimal knot of $\iograph$.
%
%VERSION 2
Minimal knot of $\iograph$ are the graphs induced by minimal knots of $\cigof\iograph$.
\end{lemma}

%\begin{proof}
%  By contradiction.
%  Let $\core = \coreof\knot$.
%  Suppose there is a proper subgraph $\coreprime$ of $\core$ which is a knot, 
%  i.e., $\gsedgesof{\coreprime} = \gsedgesof{\core} \setminus X$
%  where $X$ is non-empty.
%  Straight paths between cut-points of $\iograph$ (and inner nodes of these
%  paths) are enforced by the presence of respective cut-points and
%  Property~\ref{enum:one_path} of a closure, therefore we need to remove some
%  cut-points of $\iograph$ from $\core$.
%  Suppose we remove a set $N$ of cut-points of $\iograph$ (and all sub-edges
%  such that the result is a knot) from $\core$.
%  Then, by the correspondence between a knot in $\cigof{\iograph}$ and its
%  interpretation, $\coreprime$ is induced by a knot of
%  $\cigof{\iograph}$ which is a proper subgraph of $\knotprime$ in
%  $\cigof{\iograph}$. This is a contradiction, because $\knotprime$ is minimal.
%  $\cigof{\iograph}$?}
%  \qed
%\end{proof}
Lemma~\ref{lemma:minknot_induces_minknot} gives a way of finding minimal knots of $\iograph$ by finding minimal knots $\knotprime$ of $\cigof\iograph$ and computing cores of their interpretations by removing potential access traces. 

For instance, in Fig.~\ref{fig:igraph}, a minimal knot of $\cigof{\iographof\graph 1}$ is its subgraph $\knot'$ with $\domof\knotprime = \{2,3\}$ containing the two sub-edges of $\cigof{\iographof\graph 1}$ connecting $2$ with $3$. Node $2$ is the only source of $\knotprime$.
The interpretation $\interp$ of $\knot'$ has $\domof\interp = \{2,\bullet,3\}$ and contains all sub-edges of $\graph$ connecting the nodes $2$, $\bullet$, and $3$. Node $2$ is the source of $\interp$, $\forkof\interp 2 = \bullet$, and the sub-edge leading from $2$ to $\bullet$ is the access path of $\interp$. The highlighted area is the core $\coreof\interp$ of $\interp$, it is a minimal knot $\knot$ induced by $\knot'$, with the only source $\bullet$.
\begin{lemma}\label{lemma:disjoint_cores}
%  Given an io-graph $\iograph$ and a minimal knot $\knotprime$ of its skeleton, all cores induced by $\knotprime$ have pairwise disjoint sets of sub-edges.
  Minimal knot of $\iograph$ induced by the same minimal knot of $\cigof\iograph$ have disjoint sets of sub-edges. 
\end{lemma}

%\begin{proof}
%  First, consider a~minimal knot $\knotprime$ of $\cigof{\iograph}$ other than
%  the knot in Fig.~\ref{fig:self-loop} (note that the knot in
%  Fig.~\ref{fig:self-loop} is minimal and as such cannot be contained in any
%  other minimal knot of $\cigof{\iograph}$).
%  If $\knotprime$ is such a~knot, there is exactly one interpretation of
%  $\knotprime$ (and therefore one core induced by $\knotprime$),
%  which is due to Property~\ref{enum:one_path} of a~closure that claims that
%  there are all straight traces between nodes of $\knotprime$.
%
%  Second, for the case of the minimal knot of $\cigof{\iograph}$ in
%  Fig.~\ref{fig:self-loop}, if there is a single straight trace $\pth$ from $v$
%  to $v$, then the sub-edges of $\pth$ define a minimal knot of $\iograph$ (if
%  any sub-edge is removed, the resulting graph does not satisfy
%  Property~\ref{enum:contains_join}).
%  In the case there are multiple straight traces (i.e.~multiple cycles going
%  through $v$), then they are either disjoint (in this case the cores they
%  define are disjoint), or they have some shared sub-edges (which are at the
%  beginnings of the traces, otherwise they would traverse a cut-point) then
%  fork and finally converge in $v$.
%  In the latter case, again due to Property~\ref{enum:one_path} of a~closure,
%  the two traces will be together in one knot.
%  \qed
%  %
%  \begin{wrapfigure}[3]{r}{12mm}
%%  \vspace{-13.5mm}
%  \begin{center}
%\figswitch{
%  \hspace{-3mm}\parbox{23mm}{\input{figs/self-loop.tikz}}\\
%}
%  \vspace{-2mm}
%    \label{fig:self-loop}
%  \end{center}
%  \end{wrapfigure}
%\end{proof}

%A consequence of Lemma~\ref{lemma:disjoint_cores} is that the order in which we fold knots is arbitrary.
A consequence of Lemma~\ref{lemma:disjoint_cores} is that the order of folding minimal knots induced by a single minimal knot of does not influence the final result.

\paragraph{Arms.}
Sometimes, we will have to enlarge the found minimal knots in order to be able to fold an infinite number of them into a single box.
Given a minimal knot $\knot$ of $\iograph$, 
an \emph{arm} of $\knot$ is a tree $\tree$ with $\tree\subgraph\graph$ that contains no cut-points
of $\iograph$, with the possible exception of $\rootof{\tree}$, and every node
$v\in\domof{\tree}$ has all possible sub-edges, i.e., $\vsedgesof{\tree}
v = \vsedgesof{\graph} v$.
%A \emph{bratknot} of $\knot$ is
%a knot $\knotprime$ of $\iograph$ such that $\gsedgesof\knotprime
%= \gsedgesof\knot\cup\gsedgesof{\tree_1}\cup\cdots\cup\gsedgesof{\tree_n}$
%where each $\tree_i$, $1\leq i \leq n$, is an arm. 
%
%a tree that contains no cut-points
%of $\iograph$, with the possible exception of $\rootof{t_i}$, and every node
%$v\in\domof{\tree_i}$ has all possible sub-edges, i.e., $\vsedgesof{\tree_i}
%v = \vsedgesof{\graph} v$.
%The trees $\tree_1,\dots,\tree_n$ are called \emph{arms} of $\knot$. We note
%that a bratknot of $\knot$ may contain only arms with roots in $\knot$.
%
Our folding algorithm will sometimes fold knots together with some of their arms. The motivation for this is illustrated by the following example. 

\begin{wrapfigure}[8]{r}{24mm}
\vspace{-10mm}
\begin{center}
\figswitch{
\hspace{-3mm}\parbox{23mm}{\input{figs/csll_of_sll.tikz}}\\
}
\vspace{-2mm}
  \caption{A cyclic list of SLLs}
  \label{fig:csll_of_sll}
\end{center}
\end{wrapfigure}
%
Consider a set $C$ of all cyclic lists of singly linked lists (an example of a shape from this set is in Fig.~\ref{fig:csll_of_sll}).
Their minimal knots contain only the upper level cyclic lists (coloured in blue) and do not contain the lower level singly linked lists.
The lower level lists are arms of the cyclic lists.
Ports $\gportsprime$ of minimal knots of shapes from $C$ are elements of the border, and thus all nodes of the minimal knots (since every node is connected to a lower level singly linked list).
Since the set contains cyclic lists of an unbounded length, we are obtaining io-graphs with an unbounded number of ports and we would need to use infinitely many boxes to fold them.
However, if we fold the minimal knots including the lower level singly linked lists, the size of border will remain constant (typically 1 if one node of the cyclic list is referenced from the outside by a pointer).
The entire set $C$ can then be represented by a single box (with one port). 

\begin{wrapfigure}[3]{r}{26mm}
\vspace{-13mm}
\begin{center}
\figswitch{
\hspace{-0mm}\parbox{26mm}{\input{figs/dll.tikz}}\\
}
\vspace{-2mm}
  \caption{DLL}
  \label{fig:dll_knots}
\end{center}
\end{wrapfigure}
%
On the other hand, we cannot afford to simply always include all arms of minimal knots.
This is illustrated by an example of a set of all doubly linked lists of some type (see Fig.~\ref{fig:dll_knots}).
A strategy which would always include all arms of minimal knots could generate an infinite hierarchy of knots where every knot encodes one DLL of a certain length, in the form of the head doubly linked with another knot encoding the tail.
Similarly as in the cases of lists with head and tail pointers, this would lead to generating infinitely many nested boxes.
In this case, it is desired to fold only truly minimal knots which correspond to doubly linked list segments.

We have seen two practical situation which require opposing strategies for (not)fol-ding arms together with minimal knots. 
%Whether or not to append arms to a minimal knot to be folded therefore depends on the particular situation.
The procedure for deciding which arms to append, which we describe in Section~\ref{sec:folding_overview}, is driven by the structure of the particular FA.
Generally speaking, its goal is to include a minimal (possibly empty) set of arms so that that the resulting knots have borders of the same size and can be therefore folded into a single box. 

%Fig.~\ref{fig:tree_root_ptrs} shows an example of the io-graph $\iographof{\graph}{\bullet}$ for a tree with root pointers (with $\bullet$ as the root).
%The skeleton $\cigof{\graph}$ of this graph consists only of $\bullet$ and two looping sub-edges representing multiple cycles through $\bullet$.
%There are two minimal knots (each corresponding to one of the two sub-edges) with the same three interpretations represented by the coloured subgraphs in Fig.~\ref{fig:tree_root_ptrs}.
%



\achtung{Crossing this point disrupts integrity of space!}


%===============================================================================
\vspace*{-2mm}\subsection{Knots of Graphs}\label{sec:knots}\vspace*{-1mm}
%===============================================================================
Before we come to the details of the technique of folding FA, 
we discuss the criteria that the subgraphs of graphs of $\fa$ we consider suitable for folding into a box $B$ should satisfy.
We will investigate a strategy for picking the subgraphs to be folded
that will allow us to eliminate a large number of joins with a small number of boxes.  

A \emph{subgraph} of a graph $\graph$ 
is a graph $\graph'$ with $\domof{\graph'} \subseteq\domof{\graph}$ 
where for each $v\in \domof {\graph'}$, 
$a(v_1\cdots v_n)$ is an edge-term of $v$ in $\graph'$ 
iff (\emph{i}) it is an edge-term of $v$ in $\graph$ and (\emph{ii})
for all $1\leq i\leq n$, $v_i\in \domof{\graph'}$.
The \emph{border} of $\graph'$ in $\graph$, denoted $\borderof {\graph'} \graph$, is the subset of nodes of 
$\domof{\graph'}$
that are connected with nodes in $\domof{\graph}\setminus\domof{\graph'}$ 
by an incoming or an outgoing edge. 

We now aim at defining suitable subgraphs $\hgraph$ of a graph $\graph$ to be
folded into a box.  Let $\graph'$ be the graph that arises from $\graph$ by
folding $(\hgraph,\gports)$ into $\etermof  v i$ for some $\gports$. 

%-------------------------------------------------------------------------------
\vspace*{-1.5mm}\paragraph{Knots.}
%-------------------------------------------------------------------------------

\begin{wrapfigure}[6]{r}{0.2\textwidth}
\begin{center}
\vspace{-12mm}
\input{figs/knot.tex}
\vspace{-3mm}
  \caption{Two knots.}\label{fig:knot}
\end{center}
\end{wrapfigure}
The criteria that we see as the most crucial for selecting subgraphs to be folded are the following. 
First, to be closer to eliminating some of the joins of $\graph$ after folding, the overall sum of in-degrees of joins in the resulting graph $\graph'$ should be smaller than in the original graph $\graph$. 
The folded subgraph $\hgraph$ must hence contain at least one join of $\graph$ whose in-degree in $\hgraph$ is at least 2, or the in-degree in $\hgraph$ is 1 and $\hgraph$ contains a cycle on the join. 
Second, we require that folded graphs are accessible from some element 
of its border  
for the two following reasons: (1) we need the boxes on edge-terms of FA to be canonicity respecting, 
which is possible only if io-graphs from their languages are accessible, and (2)
accessibility of the folded subgraphs helps to eliminate counter-intuitive phenomena such as that a graph $\graph'$ is connected and the graphs in $\semof{\graph'}$ are not.
These requirements lead us to the definition of a ``knot'', a~subgraph of $\graph$ which is a candidate for folding.

A subgraph $\knot$ of $\graph$ is a \emph{knot} of $\graph$ iff
it has a node $\src\in\borderof\knot\graph$, called the \emph{source of $\knot$}, such that all nodes of $\knot$ are reachable from it and there is a join $\join\in\domof\knot$ of $\graph$ such that its in-degree in $\knot$ is at least 2 or $\join=\src$ and there is a cycle through $\join$ in $\knot$. Fig.~\ref{fig:knot} shows two knots where the source is the node with in-degree 0. 
The coloured subgraphs are ``minimal knots'' discussed in the next paragraph.

%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
\enlargethispage{6mm}
%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!

%-------------------------------------------------------------------------------
\vspace*{-1.5mm}\paragraph{Minimal knots.}
%-------------------------------------------------------------------------------

A graph may contain many knots, some of them overlap or are subgraphs of each
other. The choice of the knot to be folded is motivated by the fact that in
order to allow for encoding of sets of graphs with an unbounded number of joins
using a~finite set of boxes only, we need to learn boxes that are \emph{reusable}.  
%that encapsulate repetitive graph patterns. 
We thus aim at folding subgraphs that are likely to correspond to repetitive
graph patterns. 
%
Here,~it~is~intuitive to prioritize smaller subgraphs as they repeat more likely than complex ones, 
%subgraph has a higher chance to be reusable if it is simple.
and joins that can be eliminated by folding a large knot may usually be
eliminated by folding several smaller and simpler knots too. Second, we want folding to simplify the structure of the graph $\graph$, which intuitively means that we aim at learning boxes that interconnect as few nodes of $\graph$ as possible. That is, they enclose subgraphs with small borders.
%Folding is also simpler in the case when
%Therefore, the we seek knots that are as simple as possible. 

Hence, we define the \emph{signature} of a knot $\knot$ in a graph $\graph$ as the set $\sigof{\knot} = \joinsof\knot \cup \borderof\knot\graph$, and we
say that $k$ is \emph{simpler} than another knot $\knot'$ of $\graph$, written as $\knot \leq \knot'$, 
iff 
({\it i}) $\sigof{\knot} \subseteq \sigof{\knot'}$,  
({\it ii}) $\domof{\knot} \subseteq \domof{\knot'}$, and 
({\it iii}) every edge-term of a node $v$ in $\knot$ is also an edge-term of $v$ in $\knot'$, formally, $\forall v\rightarrow S\in\knot$, $S\subseteq S'$ where $v\rightarrow S'\in\knot'$.
We define a \emph{minimal knot} of a set of knots $\kset$ of $\graph$ as a greatest lower bound of the poset $(K, \leq)$.
In Fig.~\ref{fig:knot}, the minimal knots are coloured. %Their complexities are 2 for the knot on the top and 1 for the knot on the bottom.
%The black nodes are the entries from the sources of the nodes with indegree 0 to the set containing the only join.

%-------------------------------------------------------------------------------
\vspace*{-1.5mm}\paragraph{Optimal knots.}
%-------------------------------------------------------------------------------

We could now base the method for folding and learning boxes on the notion of minimal knots.
However, we notice that in many shape graphs created by real-life pointer programs, other than the minimal knots are the best to fold. 

\begin{wrapfigure}[11]{r}{27mm}
\vspace{-8mm}
%\begin{center}
\hspace{-3mm}\parbox{1cm}{\input{figs/root_ptr_tree.tikz}}\\
\vspace{1mm}
\hspace{1.5mm}\input{figs/sll_tail_ptr.tikz}
\vspace{-5mm}
  \caption{Minimal vs.~optimal knots.}
  \label{fig:optimal}
%\end{center}
\end{wrapfigure}
One such situation is when for a knot $\knot$, there is a node $u$, called an \emph{outer connection} of $\knot$, that reaches two nodes $v$ and $w$ of $\knot$ by straight paths. Both $v$ and $w$ must be joins since they are also reached from the source of $\knot$. 
Such a situation appears at the bottom of Fig.~\ref{fig:optimal}. It shows a list with tail pointers where the two left-most nodes are outer connections of the minimal knot, which is the subgraph containing the two right-most nodes.

At least one of the nodes $v$ and $w$, say $v$, becomes a successor of the source of the knot by the edge created when $\knot$ is folded (the other one could be its source). It will be at the same time still reached by the straight path from $u$. This means that the join $v$ cannot be eliminated unless also $u$ and the path from $u$ to it is enclosed together with $\knot$ in a box. This motivates us to fold knots that do not have any outer connections.  

Another such situation arises when there are multiple minimal knots with the same signature that always appear together. For instance,
in the case of a tree with root pointers in Fig.~\ref{fig:optimal}, the minimal knots contain the left or the right subtree and the root. To simplify the operation of folding and decrease the number of boxes, we would like to unite the two minimal knots and fold the entire tree.

Motivated by the above, we fold \emph{optimal knots}. Let $K$ be the set of knots that are minimal between those of $\graph$ that do not have any outer connections. Optimal knots are unions of knots of $K$ with the same signatures.  
Optimal knots often coincide with minimal knots as is the case in Fig.~\ref{fig:knot}.  
This is, however, not the case of Fig.~\ref{fig:optimal} where optimal knots are the entire tree and the entire list (depicted in blue with a solid outline).


%-------------------------------------------------------------------------------
\paragraph{Finding optimal knots in a graph.}
%-------------------------------------------------------------------------------
We now study some simple properties of optimal knots which allow us to detect them in a graph $\graph$, and which will in turn allow us to detect substructures of FA that accept optimal knots. 
We first observe that optimal knots are uniquely identified by their signatures, as will be stated by the lemma below.  
%We first observe that for a given signature, there exists (at most) one unique optimal knot.  

Let $u,v$ be nodes of $\graph$. A \emph{tree segment} $t$ between $u$ and $v$ is a subgraph of $\graph$ such that it contains a straight path $\pth$
from $u$ to $v$, all straight paths from inner nodes of $\pth$ to the leaves of $\graph$, and there is no proper subgraph of $t$ with this property.
%
\begin{lemma}\label{lemma:signature}
Let $V\subseteq\domof\graph$ and $\knot$ be the optimal knot of $\graph$ with the signature $V$.
Then $k$ is the smallest subgraph of $\graph$ that contains all tree segments
between the nodes of $V$. 
\end{lemma}
%
Next, we observe that elements of signatures of optimal knots are joins of the graph $\graph$, possibly with the exception of their sources.  

We define the notion of \emph{entry} of $u\in\domof\graph$ to $V\subseteq\domof\graph$ in a graph $\graph$, denoted $\entryof \graph u V$,
as the node $\entry$ which equals $u$ in case there is a straight path from some node in $V$ into $u$, and otherwise it is the node which has the property that
all straight paths from $u$ to
$V$ traverse it and no successor of $e$ has this
property. 

\begin{lemma}\label{lemma:joins}
The signature of an optimal knot of $\graph$ is a set 
$J\setminus\{\join\}\cup\{\entry\}$ where 
$J\subseteq\joinsof\graph$,
$\join\in J$,
and $\entry = \entryof \graph \join J$ is its source. 
\end{lemma}
%
The following lemma suggests that signatures of optimal knots of $\graph$ correspond almost precisely (up to the sources of the knots) to signatures of optimal knots of 
the interconnection graphs of $\graph$ that contain all joins of $\graph$. 

\begin{lemma}\label{lemma:igraph}
There is an optimal knot in $\igraphof \graph V$ such that $\joinsof\graph\subseteq V\subseteq \domof\graph$ 
with a signature $J$ and a source $\src\in J$
iff
there is an optimal knot of $\graph$ with the signature $J\setminus\{\src\}\cup\{\entry\}$ where $\entry = \entryof\graph\src J$ is its source.
\end{lemma}
%
We say that the signature $J$ of the optimal knot in $\igraphof \graph V$ from the above lemma \emph{approximates} the signature $J\setminus\{\src\}\cup\{\entry\}$, and that $J\setminus\{\src\}\cup\{\entry\}$ \emph{concretizes} $J$ in $\graph$.

Lemma~\ref{lemma:igraph} is illustrated in Fig.~\ref{fig:igraph}.
The set $J = \{1,3\}$ is the signature of an optimal knot  in $\cigraphof{\graph,1}$ (the subgraph of $\cigraphof{\graph,1}$ with the domain $\{1,3\}$ and the two edge-terms connecting $1$ to $3$) with the source $\src = 1$.
The entry $\entry = \entryof \graph \src J$ of $1$ to $\{3\}$ in $\graph$ is the black node $\bullet$.
The concretization of $\{1,3\}$ is thus the set $J\setminus\{\src\}\cup\{\entry\} = \{\bullet,3\}$, which is the signature of the blue optimal knot of $\graph$ (with the source $\bullet$).

By Lemmas~\ref{lemma:signature}, \ref{lemma:joins}, and \ref{lemma:igraph}, optimal knots of $\graph$ can be identified by the following steps:
\begin{enumerate}
\item
Start from the signature $J$ of some optimal knot of $\igraphof \graph V$ with $\joinsof\graph\subseteq V\subseteq \domof\graph$ 
%(possibly $\cigraphof{\graph,\gports}$ for an io-graph $(\graph,\gports)$)
%(it can possibly be the cut-point interconnection graph of an io-graph) 
(e.g., a cut-point interconnection graph)
with the source $\src\in J$.
\item
Find a concretization $J$ in $\graph$ as the signature $J\setminus\{\src\}\cup\{\entry\}$ where $\entry=\entryof\graph\src J$.
\item
Construct the optimal knot in $\graph$ as the smallest subgraph of $\graph$ containing all tree segments between nodes of $J\setminus\{\src\}\cup\{\entry\}$.
\end{enumerate}

